Asynchronous Sessions with Input Races

We propose a calculus for asynchronous multiparty sessions where input choices with different senders are allowed in processes. We present a type system that accepts such input races provided they do not hinder lock-freedom.

==> eptcsdata.tex <==
\providecommand{\firstpage}{12}
\providecommand{\publicationstatus}{M. Carbone and R. Neykova (Eds.): 13th International\\
Workshop on Programming Language Approaches to\\
Concurrency and Communication-cEntric Software\\
EPTCS 356, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.356.2}{10.4204/EPTCS.356.2}}

